A Local to Global Principle for the Complexity of Riemann Mappings (Extended Abstract)

We show that the computational complexity of Riemann mappings can be bounded by the complexity needed to compute conformal mappings locally at boundary points. As a consequence we get first formally proven upper bounds for Schwarz-Christoffel mappings and, more generally, Riemann mappings of domains with piecewise analytic boundaries.

==> eptcsdata.tex <==
\providecommand{\event}{X. Zheng and N. Zhong (Eds.)\\
Computability and Complexity in Analysis (CCA 2010)}
\providecommand{\volume}{24}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{120}
\providecommand{\eid}{16}

